Interacting Barrow Holographic Dark Energy in Non-flat Universe

Barrow holographic dark energy model is an extension of holographic dark energy that incorporates modifications to entropy due to quantum gravitational effects. In this work we study the cosmological properties of interacting Barrow holographic dark energy model in the case of non-zero curvature universe. We construct the differential equations governing the evolution of the Barrow holographic dark energy density parameter and the dark matter density parameter in coupled form for both closed and open spatial geometry. Considering three different forms of coupling, we obtain the corresponding analytical expressions for the equation of state parameter for the dark energy component. We confront the scenario using recent observational datasets like cosmic chronometer and Pantheon data. It has been found that the strength of interaction as well as the curvature contribution come out to be nonzero which indicates that a non-flat interacting scenario is preferred by observational data.

==> packages.tex <==
\usepackage{etex}
\reserveinserts{28}

\usepackage{aybufbe}

\usepackage[utf8]{inputenc}
\usepackage{dsfont}
\usepackage{txfonts}
\usepackage{pstricks,pst-node,pst-text,pst-3d}
%\usepackage[round,comma]{natbib} %apa için bu aktif olmalı
\usepackage{vmargin}
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{epstopdf}
\usepackage{float}
\usepackage{verbatim}
%\usepackage{caption}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{url}

\usepackage{cite} %apa için deaktif olmalı


\usepackage{mathtools}

\usepackage{longtable}
\usepackage{nomencl}

%\usepackage[unicode]{hyperref}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{rotating}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{mathrsfs}
\usepackage{tikz}
\usepackage{comment}
\usepackage{dblfloatfix}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{tablefootnote}
\usepackage{booktabs}
%if you do not need, comment them
\usepackage{subcaption}
\usepackage{siunitx}
\usepackage{array}
\usepackage{amsmath}

%\usepackage[%labelsep=newline,%font=bf,%labelfont =bf,%textfont = bf,justification=centering]{caption}
\usepackage[justification=centering]{caption}
\usepackage{setspace}
\usepackage{fancyhdr}
\usepackage{etoolbox}
\usepackage{tabularx}

\usepackage{calc}

\usepackage{hyperref}
\hypersetup{colorlinks=false, unicode=true, citecolor=black, filecolor=black, linkcolor=black, urlcolor=black, anchorcolor=black, hidelinks, linktoc=all}
%\usepackage{hyperref} %%pdflatex degil de latex yapiliyorsa bunu kullan, dvi bakmak icin yapta problem olursa
%%%%% you can change the color of hyperlinks %%%%
%\renewcommand{\chapterautorefname}{Chapter}

\usepackage[nameinlink]{cleveref}

%% Birden çok satırlı başlıkların ilk satır dışında kalan kelimeleri numara ile aynı yerden başlasın diye gerekli kod
\makeatletter
\def\@hangfrom#1{\setbox\@tempboxa\hbox{{#1}}%
      \hangindent 0pt%\wd\@tempboxa
      \noindent\box\@tempboxa}
\makeatother

%% Contents'te noktaların numaralar kadar tam gitmesi için
\makeatletter
\renewcommand{\@pnumwidth}{0pt{}}% 40pt is just an example
\makeatother

%%%%%%%%%%%%%%%%%%% NOMENCLATURE %%%%%%%%%%%%%%%%%%%%

\makenomenclature

\renewcommand{\nomname}{}
\renewcommand{\nompreamble}{\vspace*{-7mm}} % title sonrası bosluk
%\setlength{\nomlabelwidth}{1.5cm} % bunu eğer uzun bir kısaltma olup yazıya dokunuyorsa düzenle
\setlength{\nomitemsep}{-\parsep}


\renewcommand\nomgroup[1]{%
  \item[\bfseries
  \ifstrequal{#1}{D}{Acronyms}{%
  \ifstrequal{#1}{B}{Greek Letter Symbols}{%
  \ifstrequal{#1}{A}{Roman Letter Symbols}{
  \ifstrequal{#1}{C}{\hspace{-1mm}Subscripts}{}}}}
  ]}
% -----------------------------------------

%%%%%%%%%%%%%%%%%%% NOMENCLATURE DONE %%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
%\usepackage[backend=biber,style=apa,babel=other,maxcitenames=6]{biblatex}

%%% Colors %%%%%
\definecolor{OvGUMEMoRIAL}{HTML}{F7DB2B}
\definecolor{ISDUE}{HTML}{475BF9}
\definecolor{lachinov}{HTML}{347AFD}
\definecolor{IITKGP-KLIV}{HTML}{463DE0}
\definecolor{MedianCHAOS1}{HTML}{2797EB}
\definecolor{MedianCHAOS2}{HTML}{17AEDA}
\definecolor{MedianCHAOS3}{HTML}{12BEB9}
\definecolor{MedianCHAOS4}{HTML}{3DC990}
\definecolor{MedianCHAOS5}{HTML}{81CC59}
\definecolor{MedianCHAOS6}{HTML}{C8C129}
\definecolor{PKDIA}{HTML}{F9FB15}
\definecolor{mountain}{HTML}{FCBB3E}
\definecolor{CIR-MPerkonigg}{HTML}{3E26A8}
\definecolor{PKDIAv2}{HTML}{F9FB15}
\definecolor{METU_MMLAB}{HTML}{FF0000}
\definecolor{nnU-Net}{HTML}{F72A9B}
\newcommand{\teamcolor}[1]{
\begin{tikzpicture}
\draw [fill=#1, draw=#1]circle (1.0mm);
\end{tikzpicture}}
\usepackage{soul}
\newcommand{\note}[1]{\textcolor{red}{#1}}

% Kurallar

\newlength\myindention
\DeclareCaptionFormat{mytable}%
{\hspace*{\myindention}#1#2#3}
\setlength\myindention{-0.5cm}

\theoremstyle{plain}
%\theoremstyle{property}
\newtheorem{property}[theorem]{Property}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Caption settings in figures and tables

\makeatletter
\patchcmd{\@caption}{\csname the#1\endcsname}{\csname fnum@#1\endcsname\hfill \ \ \ }{}{}
%\renewcommand*\l@figure{\@dottedtocline{1}{1.5em}{4.5em}} % default for 3rd arg: 2.3em

\let\l@table\l@figure % as in article.cls
\makeatother
\captionsetup{format=plain, font=small, labelfont=bf}
\captionsetup[figure]{labelsep=space, singlelinecheck=true, font=footnotesize,justification=centering}
%\captionsetup[figure]{labelsep=space, singlelinecheck=false, font=footnotesize,justification=justified}
\captionsetup[table]{labelsep=space, singlelinecheck=false, font=footnotesize,justification=centering}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Equation Cite settings   %%%%%%%%%%%%%%%%%%%
\makeatletter
\def\tagform@#1{\maketag@@@{\normalfont(\ignorespaces#1\unskip\@@italiccorr)}}
\renewcommand{\eqref}[1]{\textup{{\normalfont\autoref{#1}}\normalfont}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Hyphenation settings   %%%%%%%%%%%%%%%%%%%
\tolerance=1% 
\emergencystretch=\maxdimen%
\hyphenpenalty=10000%
\hbadness=10000

%%%%% Çoklu kaynaklar arası noktalı virgül %%%%%%
%\usepackage{etoolbox} %2. kez tanım, line 49
\makeatletter
\newcommand\bibstyle@semicolon{\bibpunct();a,,}
\makeatother

%%%%% Section titleı için sayı ile text arası mesafe %%%%%%
\makeatletter
\renewcommand*{\@seccntformat}[1]{\csname the#1\endcsname\hspace{1mm}}
\makeatother

%apa için aktif olmalı
%\pretocmd\citep{\citestyle{semicolon}}\relax\relax
%\pretocmd\Citep{\citestyle{semicolon}}\relax\relax
%%%%% Çoklu kaynaklar arası noktalı virgül %%%%%%

%%% Sayfa boyutları %%%%%%%

\setlength{\paperheight} {297mm}
\setlength{\paperwidth } {210mm}
\setlength{\oddsidemargin} {0mm}
\setlength{\evensidemargin} {0mm}
\setlength{\marginparwidth} {0mm}
\setlength{\marginparsep} {0mm}
\setlength{\topmargin} {-12mm}
\setlength{\headheight} {6.89pt} %0mm, in order to remove the warning
\setlength{\headsep} {12mm}%%tepeden
\setlength{\voffset}{0mm}
\setlength{\hoffset}{14.75mm}
\setlength{\textheight} {242mm} %3+3=6cm cıkmıs hali 237mm
\setlength{\textwidth} {145mm} %4+2.5=6.5cm cıkmıs hali 145mm
\setlength{\footskip}{35pt}  %%%%  page number position

%\usepackage{geometry}
 %\geometry{
% left=40mm,
% top=30mm,
% }
\renewcommand{\chapterautorefname}{Chapter}
%%% Sayfa boyutları %%%%%%%
%aet
